MINT: Securely Mitigating Rowhammer with a Minimalist In-DRAM Tracker

This paper investigates secure low-cost in-DRAM trackers for mitigating Rowhammer (RH). In-DRAM solutions have the advantage that they can solve the RH problem within the DRAM chip, without relying on other parts of the system. However, in-DRAM mitigation suffers from two key challenges: First, the mitigations are synchronized with refresh, which means we cannot mitigate at arbitrary times. Second, the SRAM area available for aggressor tracking is severely limited, to only a few bytes. Existing low-cost in-DRAM trackers (such as TRR) have been broken by well-crafted access patterns, whereas prior counter-based schemes require impractical overheads of hundreds or thousands of entries per bank. The goal of our paper is to develop an ultra low-cost secure in-DRAM tracker. Our solution is based on a simple observation: if only one row can be mitigated at refresh, then we should ideally need to track only one row. We propose a Minimalist In-DRAM Tracker (MINT), which provides secure mitigation with just a single entry. At each refresh, MINT probabilistically decides which activation in the upcoming interval will be selected for mitigation at the next refresh. MINT provides guaranteed protection against classic single and double-sided attacks. We also derive the minimum RH threshold (MinTRH) tolerated by MINT across all patterns. MINT has a MinTRH of 1482 which can be lowered to 356 with RFM. The MinTRH of MINT is lower than a prior counter-based design with 677 entries per bank, and is within 2x of the MinTRH of an idealized design that stores one-counter-per-row. We also analyze the impact of refresh postponement on the MinTRH of low-cost in-DRAM trackers, and propose an efficient solution to make such trackers compatible with refresh postponement.

==> rebuttal.tex <==
\clearpage

\section*{Rebuttal and Revision Log}

We thank the reviewers for feedback.  We have revised the paper to address the concerns (changes marked in \textcolor{blue}{blue}). We first address the common concern and then reviewer questions.

\vspace{0.05 in}
\noindent{\bf{COMMON-1: MINT is similar to Single-Entry PARA}}
\vspace{0.05 in}

\noindent This seems to be a {\bf{major}} misunderstanding. To highlight the differences between InDRAM-PARA and MINT, we add a new section (Sec-III: Pitfalls of InDRAM-PARA) that shows the shortcomings of InDRAM-PARA that MINT addresses. MINT has  2.7x lower threshold and better security than InDRAM-PARA. We replace the term {\em IID-Tracker} with InDRAM-PARA for clarity. We urge the reviewers to check out Section-III. 


\vspace{0.05 in}
\noindent{\bf{COMMON-2: In-DRAM PARA can be made secure by avoiding overwrite of stored row (Rev-D and Rev-E)}}
\vspace{0.05 in}

\noindent While this solution seems intuitive, it is equally vulnerable to our InDRAM-PARA design. It suffers from non-uniform sampling. The last row in tREFI interval now becomes the most-vulnerable one as it cannot be selected if ANY of the prior rows got selected. We describe the pitfalls of this design in Section III-B. It has 2.7x higher threshold compared to MINT.  We note that this well-meaning suggestion from two {\em expert} reviewers is ineffective, which further highlights that it is quite challenging to apply PARA to in-DRAM setting, and that MINT is not a minor variation of PARA.


%that MINT cannot be deemed a minor variation of PARA.


\vspace{0.05 in}
\noindent{\bf{COMMON-3: DMQ is Simple and Obvious }}
\vspace{0.05 in}

\noindent  Prior low-cost trackers were insecure and could be broken easily with simple patterns, so there was no need for refresh-postponement attacks or DMQ. As refresh-postponement is a new attack vector, we developed the DMQ solution. Indeed, our aim was to develop a simple and effective solution, as such solutions are more likely to get adopted within DRAM. Note that simplicity does not mean a lack of novelty or creativity.

\vspace{0.1 in}
\noindent{\bf{=============== Reviewer-A ================}}
\vspace{0.1in}

Per feedback, we moved Appendix-A to the new Section-III.

%to highlight the shortcomings of InDRAM-PARA. 

\vspace{0.05 in}
\noindent {\bf{1. Can attacker precisely sync up with the refresh interval?}} Yes, Refresh-Interval-Synchronization is already a popular technique for Rowhammer attacks. For example,  SMASH~\cite{de2021smash} and BlackSmith~\cite{jattke2021blacksmith} used it to break TRR. 

\vspace{0.05 in}

\noindent  \noindent {\bf{2. Attackers aim should be to maximize the success per unit time. Attacker can reattempt (explain Figure-6)?}} Indeed. The reviewer seems to misunderstand our methodology. Our MinTRH evaluations assume the pattern runs continuously. Fig-6 shows the MinTRH of MINT, derived for mean-time-to-failure if Pattern-3 runs continuously for thousands of years.

\vspace{0.05 in}

\noindent {\bf{3. DMQ obvious, if DDR5 queues up refreshes? }} Please see COMMON-3. Also, the memory controller postpones refreshes by delaying the sending of the refresh pulse, the DDR5 chip does not ``queue up" anything for postponement.


\vspace{0.1 in}
\noindent{\bf{=============== Reviewer-B ================}}
\vspace{0.1in}

\noindent {\bf{1. Vary DDR5 Parameters:}}  See newly added Appendix-A. Benefit of MINT is similar over the entire DDR5 range. 

\vspace{0.05 in}

\noindent {\bf{2. Power Methodology:}}  We have revised Section VIII-D to provide  details of our methodology (includes RNG and DMQ).   

\vspace{0.05 in}
\noindent {\bf{3. Uniformity vs Non-Uniformity:}} Yes, see new Section-III.

\vspace{0.05 in}
\noindent {\bf{4. URAND(0,365):}} We evaluated this design. 
 As it has 5x lower mitigation probability than MINT, it has MinTRHD-D of 6563 (4.7x higher than MINT and 4.43x of MINT+DMQ).
 
\vspace{0.1in}
\noindent{\bf{=============== Reviewer-C ================}}
\vspace{0.1in}

\noindent Minor increment over PARA: See COMMON-1, Sec-III.

\vspace{0.05 in}
\noindent {\bf{1. Compare against PARA:}} New Sec-III compares against InDRAM-PARA (we have 2.7x lower threshold). Fig-17 compares against MC-PARA (we have 8\% lower slowdown)

\vspace{0.05 in}
\noindent {\bf{2. Row-Press?}} Row-Press depends on the  time the memory-controller (MC) keeps the row open (tON), and this time is not dependent on the choice of in-DRAM tracker (e.g. MINT). Row-Press can be solved by circuit-level techniques (Row-Buffer decoupling) or using MC to limit tON.  To the best of our knowledge, currently, there is no tracker design that can itself securely mitigate both Rowhammer and Row-Press.

%without relying on circuit-solutions or forcing MC to limit tON.




\vspace{0.1in}
\noindent{\bf{=============== Reviewer-D ================}}
\vspace{0.1in}

\noindent Incremental over PARA: Please see COMMON-1 and Sec-III


\vspace{0.05 in}
\noindent {\bf{1. Avoid Overwriting the Targeted Row?}} This design would still be insecure, please see COMMON-2. 

\vspace{0.05 in}
\noindent {\bf{2. Non-Selection in PARA:}} Agree, see Section III-D

\vspace{0.05 in}
\noindent {\bf{3. Not convinced RFM vs DRFM is fundamental limitation of PARA:}} We compare with InDRAM-PARA (uses RFM) and show that MINT has 2.7x lower threshold.  We compare against MC-PARA (uses DRFM) and show that MINT has up-to 8\% higher performance. Thus, MINT is better in both cases. 


\vspace{0.1in}
\noindent{\bf{=============== Reviewer-E ================}}
\vspace{0.1in}

\vspace{0.05 in}
\noindent {\bf{1. Why use MINT if PRAC?}} We note that PRAC specifications were released a few hours before the submission deadline, so we could not discuss.  Nonetheless, PRAC requires significant area (Hynix reports 9\%) and timing (tRC increase by 10\%). DDR5 specifies that PRAC is an OPTIONAL feature and DRAM vendors can choose to not support it. DRAM is a cost-sensitive market, so if there is secure low-cost solution to mitigate Rowhammer, such a solution is more likely to get used than PRAC. MINT offers such a practical alternative. 

\vspace{0.05 in}
\noindent {\bf{2. MINT similar to single-entry PARA:}}  See COMMON-1. 


\vspace{0.05 in}
\noindent{\bf{2. Secure In-DRAM PARA by Avoiding Overwrite:}}  This design would still be insecure, please see COMMON-2. 


\vspace{0.05 in}
\noindent {\bf{3. DMQ Power, Area, Logic and Timing?}} Section VIII-D now includes DMQ power (negligible, 86 micro-watts). The logic and timing of DMQ is similar to TRR, so compatible with DDR5. DMQ area is 7x lower than TRR (30 vs 4 entries).




\vspace{0.1in}
\noindent{\bf{=============== Reviewer-F ================}}
\vspace{0.1 in}

Thanks for the feedback. Please see newly added Sec-III. The ``ideal" line in Figure~\ref{fig:mitprob} (Sec-III) corresponds to MINT. 



==> spatial.tex <==


%(workloads sorted in descending order of rate of DRAM ACTs)

%\newpage

\color{red}
\section{The Impact of Victim-Sharing Attacks}
\label{sec:spatial}


The security of PrIDE stems from the guarantee that the likelihood that a row will encounter TRH* activations without getting mitigated is negligibly small (once per 1000 years). An attacker could try to launch an attack pattern that shares a victim row, as a means of causing more hammers on the shared victim row, without triggering a refresh of the victim.


\begin{figure}[h!]
    \centering
    \includegraphics[width=2.75 in]{Figures/victimshare.pdf}
   % \vspace{-0.05 in}
    \caption{Victim sharing attacks for Blast Radius of 1 and 2.}
    \label{fig:spatial}
  %  \vspace{-0.1 in}
\end{figure}




Figure~\ref{fig:spatial} shows the victim-sharing attacks for a system designed for a Rowhammer Threshold of $T$. For Blast-Radius (BR) of 1, the victim-row C is shared between aggressor rows B and D.  For BR=2, the victim-row C is shared between four aggressor rows A, B, D, and E.  If we had a counter-based mitigation~\cite{park2020graphene,kim2022mithril,ProTRR,qureshi2022hydra,CBT,lee2019twice}, such victim sharing attacks can subject the victim row to 2*(T-1) or 4*(T-1) hammers without triggering a refresh of the victim, thereby reducing the effective threshold handled by the counter-based mitigation schemes. As such victim-sharing attacks are effective in the presence of counter-based mitigations, it may seem intuitive that they are also effective against PrIDE.


We observe that PrIDE is probabilistic and causes a refresh of the shared victim-row if any of the aggressors within the BR gets selected for mitigation (mitigation refreshes BR rows on either side of the aggressor row). For example, for BR=1 attack, each activation of Row-B or Row-D can trigger a refresh of the victim Row-C. Therefore, the total number of chances the victim-row has of getting refreshed is the sum of the activation counts across all the aggressor rows within the BR.  We can view TRH* of PrIDE as the consecutive number of chances of mitigation that remain unmitigated.  Thus, with PrIDE, for BR=1 attacks, the average number of activations on the two aggressor rows can be at most half of TRH* while escaping mitigation (for BR=2 attack, the four aggressor rows can have an average activation counts of only a quarter of TRH* while escaping mitigation). Thus, PrIDE is robust against victim-sharing attacks as mitigation is proportional to the total number of hammers suffered by the victim.   

We can use this analysis to also determine the Rowhammer Threshold  (TRH-D*) tolerated by PrIDE for the double-sided rowhammer pattern (pattern is identical to BR=1 victim-sharing attack). \color{black} In the double-sided pattern,  each aggressor row is accessed TRH-D times, thus the victim row has 2*TRH-D chances of getting mitigated.  For example, if TRH-D was 4.8K, PrIDE would get 9.6K chances to refresh the victim row.  Thus, the TRH* of PrIDE can be halved for a double-sided pattern, while still retaining the same target failure rate. Table~\ref{tab:spatial} shows the single-sided (TRH-S*) and double-side (TRH-D*) thresholds tolerated by PrIDE and PrIDE+RFM. PrIDE can tolerate (the typically reported TRH) {\bf TRH-D* of 1.7K}, and PrIDE+RFM16 can tolerate {\bf TRH-D* of 367}.



\begin{table}[htb]
  \centering
    \vspace{-0.1in}
  \caption{The TRH-S* and TRH-D* of PrIDE and PrIDE+RFM}
  \label{tab:spatial}
  \begin{tabular}{ccc}
    \hline
   \textbf{Scheme} & \textbf{TRH-S* (Single-Sided)} & \textbf{TRH-D* (Double-Sided)}\\ \hline 
    PrIDE          & 3.40K   & 1.70K \\ %\hline   
    PrIDE+RFM40    & 1.76K    & 880 \\ 
    PrIDE+RFM16    & 733     & {\bf 367} \\ \hline 
  \end{tabular}
\vspace{-0.15in}
\end{table}



